Elasticity and acoustic velocities of $\delta$-AlOOH at extreme conditions: a methodology assessment

Hydrous phases play a fundamental role in the deep-water cycle on Earth. Understanding their stability and thermoelastic properties is essential for constraining their abundance using seismic tomography. However, determining their elastic properties at extreme conditions is notoriously challenging. The challenges stem from the complex behavior of hydrogen bonds under high pressures and temperatures (P,Ts). In this study, we evaluate how advanced molecular dynamics simulation techniques can address these challenges by investigating the adiabatic elasticity and acoustic velocities of $\delta$-AlOOH, a critical and prototypical high-pressure hydrous phase. We compared the performances of three methods to assess their viability and accuracy. The thermoelastic tensor was computed up to 140 GPa and temperatures up to 2,700 K using molecular dynamics with a DeePMD machine-learning interatomic potential based on the SCAN meta-GGA functional. The excellent agreement with ambient condition single-crystal ultrasound measurements and the correct description of velocity changes induced by H-bond disorder-symmetrization transition observed at 10 GPa in Brillouin scattering measurements underscores the accuracy and efficacy of our approach.

==> flowchart.tex <==
\begin{tikzpicture}[
  block/.style={
    rectangle,
    draw,
    text width=8em,
    text centered,
    minimum height=5em,
    node distance=1cm,
    inner ysep=.75em,
    inner xsep=.5em,
    font=\small,
    execute at begin node={\setlength{\baselineskip}{3ex}}
  },
  line/.style={
    draw,
    -latex'
  }
]

\small


% Nodes
\node [block] (npt) {Perform $NPT$ MD to optimize cell shape};
\node [block, right=of npt] (hp) {Calculate heat capacity $C_V$};
\node [block, below=of npt] (isothermal) {Calculate isothermal elastic tensor $C_{ij}^T$};
\node [block, below=of hp] (adiabatic) {Calculate adiabatic elastic coefficient $C_{ij}^S$};
\node [block, right=of adiabatic] (moduli) {Elastic moduli $K$, $G$ and acoustic velocity $V_S$, $V_P$};

% Lines
\draw [line] (npt) -- (hp);
\draw [line] (npt) -- (isothermal);
\draw [line] (hp) -- (adiabatic);
\draw [line] (isothermal) -- (adiabatic);
\draw [line] (adiabatic) -- (moduli);

\end{tikzpicture}
